Differential Good Arm Identification

This paper targets a variant of the stochastic multi-armed bandit problem called good arm identification (GAI). GAI is a pure-exploration bandit problem with the goal to output as many good arms using as few samples as possible, where a good arm is defined as an arm whose expected reward is greater than a given threshold. In this work, we propose DGAI - a differentiable good arm identification algorithm to improve the sample complexity of the state-of-the-art HDoC algorithm in a data-driven fashion. We also showed that the DGAI can further boost the performance of a general multi-arm bandit (MAB) problem given a threshold as a prior knowledge to the arm set. Extensive experiments confirm that our algorithm outperform the baseline algorithms significantly in both synthetic and real world datasets for both GAI and MAB tasks.

==> LaTeX/criteria-fig.tex <==
\begin{figure*}[!bth]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-synth_small.pdf}
        \caption{Synth small offline.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-synth_large.pdf}
        \caption{Synth small online.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-openbandit.pdf}
        \caption{Synth small offline.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-movielens.pdf}
        \caption{Synth small online.}
    \end{subfigure}
    
    \caption{The curve shows the difference of two different criteria during one training trajectory.}
    \label{fig:criteria-diff}
\end{figure*}

==> bound-fig.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/bound-synth_small.pdf}
        \caption{Synth small}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/bound-synth_large.pdf}
        \caption{Synth large}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/bound-openbandit.pdf}
        \caption{Openbandit}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/bound-movielens.pdf}
        \caption{MovieLens}
    \end{subfigure}
    
    \caption{Confidence bound comparison. This figure plots the identification bound for the best arm in the arm set $\mathcal{A}$ during the training trajectory and compare the difference between ours and the baselines.}
    \label{fig:bound-compare}
\end{figure*}

==> criteria-fig.tex <==
\begin{figure*}[!bth]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-synth_small.pdf}
        \caption{Synth small offline.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-synth_large.pdf}
        \caption{Synth small online.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-openbandit.pdf}
        \caption{Synth small offline.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/criteria-movielens.pdf}
        \caption{Synth small online.}
    \end{subfigure}
    
    \caption{The curve shows the difference of two different criteria during one training trajectory.}
    \label{fig:criteria-diff}
\end{figure*}

==> curve-fig.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/curve-synth_small.pdf}
        \caption{Synth small.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/curve-synth_large.pdf}
        \caption{Synth large.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/curve-openbandit.pdf}
        \caption{Openbandit.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/curve-movielens.pdf}
        \caption{MovieLens.}
    \end{subfigure}
    
    \caption{Learning curves of $\alpha,\beta$. Solid lines represent offline setting and the dash line represent online setting. The horizontal axis in offline setting is training epochs while in online setting is sampling rounds $t\in[T]$. The curve shows that the parameters converges as the training epochs goes on and it converges slower in online setting.}
    \label{fig:learning-curve}
\end{figure*}

==> diff-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Initialize:}}

\begin{algorithm}[t]


\caption{The differential algorithm to learn the optimal confidence bound for both sampling strategy and identification criteria.}

\begin{algorithmic}[1]
\label{alg:ours}

\REQUIRE $N$, $\mathcal{A}$, $K$, $T$,  $\lambda$, $\eta$
\ENSURE  $\alpha_0=0,~\beta_0=0,~V_0=I\in\mathbb{R}^{d\times d},~b_0\in\mathbb{R}^d,~\gamma_0=0$

\FOR{$n=1$ to $N$}
    \FOR{$t=1$ to $T$}
        \STATE Find $S_{i,t}, \forall i\in \mathcal{A}$ via Eq.~\ref{eq:S} with $\beta$.
        \STATE Find $P_t$ via Eq.~\ref{eq:P}.
        \STATE Select arm $i_t \in \mathcal{A}$ randomly according to $P_t$ and receive reward $y_t$.
        \STATE Update $\mathbf{V}_t\gets \mathbf{V}_{t}+\mathbf{x}_t\mathbf{x}_t^T$, $\mathbf{b}_t\gets \mathbf{b}_{t-1}+\mathbf{x}_ty_t$.
        \STATE Update $\gamma_t$ via Eq.~\ref{eq:P}.
        \STATE (Online) Update $\beta \gets \hat{\beta}_{t-1}+\lambda \nabla_\beta$, $\alpha \gets \hat{\alpha}_{t-1}+\lambda \nabla_\alpha$ via Eq.~\ref{eq:online_objective}
    \ENDFOR
    \STATE (Offline) Update $\beta \gets \hat{\beta}_{t-1}+\lambda \nabla_\beta$, $\alpha \gets \hat{\alpha}_{t-1}+\lambda \nabla_\alpha$ via Eq.~\ref{eq:offline_sample_objective_constraint} and Eq.~\ref{eq:offline_identify_objective_constraint}
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> exp1-performance-fig.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp1-synth_small.pdf}
        \caption{Synth small}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp1-synth_large.pdf}
        \caption{Synth large}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp1-openbandit.pdf}
        \caption{Openbandit}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp1-movielens.pdf}
        \caption{MovieLens}
    \end{subfigure}
    
    % \\
    
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{example-image}
    %     \caption{Synth small offline.}
    %     \label{fig:no-batch}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{example-image}
    %     \caption{Synth small online.}
    %     \label{fig:batch}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{example-image}
    %     \caption{Synth small offline.}
    %     \label{fig:no-batch}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{example-image}
    %     \caption{Synth small online.}
    %     \label{fig:batch}
    % \end{subfigure}
    
    \caption{Comparison of our proposed method with several baselines on all datasets. The cumulative exploit score shows that our proposed method outperforms the baselines in solving GAI problem as the learned confidence bound w.r.t $\alpha,\beta$ converges. The performance in online setting converges slower but also eventually outperform other baselines.}
    \label{fig:exp1}
\end{figure*}

==> exp2-performance-fig.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp2-synth_small.pdf}
        \caption{Synth small.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp2-synth_large.pdf}
        \caption{Synth large.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp2-openbandit.pdf}
        \caption{Openbandit.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{LaTeX/Figs/exp2-movielens.pdf}
        \caption{MovieLens.}
    \end{subfigure}
    
    \caption{Comparison of our proposed method with several baselines on all datasets. The cumulative reward shows that our proposed method outperforms the baselines in solving cumulative reward maximization problem as the learned confidence bound w.r.t $\alpha,\beta$ converges to optimal.}
    \label{fig:exp2}
\end{figure*}

==> hdoc-algo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}


\begin{algorithm}[t]


\caption{HDoC algorithm. The base algorithm for solving GAI problem.}

\begin{algorithmic}[1]
\label{alg:hdoc}
\REQUIRE a  $\xi$, $\delta$, $K$, $\mathcal{A}$
\STATE Pull each arm once
\FOR{$t=1$ to $T$}
    \STATE Pull arm $a^*_t$ selected by sampling strategy
    \IF{$\underline{\mu}_{a^*_t} \geq \xi$}
        \STATE Identify $a^*_t$ as good
        \STATE remove $a^*_t$ from $\mathcal{A}$
    \ENDIF
    \IF{$\overline{\mu}_{a^*_t} < \xi$}
        \STATE Identify $a^*_t$ as bad
        \STATE remove $a^*_t$ from $\mathcal{A}$
    \ENDIF
\ENDFOR

\end{algorithmic}
\end{algorithm}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
